SSCAP: Self-supervised Co-occurrence Action Parsing for Unsupervised Temporal Action Segmentation

Temporal action segmentation is a task to classify each frame in the video with an action label. However, it is quite expensive to annotate every frame in a large corpus of videos to construct a comprehensive supervised training dataset. Thus in this work we propose an unsupervised method, namely SSCAP, that operates on a corpus of unlabeled videos and predicts a likely set of temporal segments across the videos. SSCAP leverages Self-Supervised learning to extract distinguishable features and then applies a novel Co-occurrence Action Parsing algorithm to not only capture the correlation among sub-actions underlying the structure of activities, but also estimate the temporal path of the sub-actions in an accurate and general way. We evaluate on both classic datasets (Breakfast, 50Salads) and the emerging fine-grained action dataset (FineGym) with more complex activity structures and similar sub-actions. Results show that SSCAP achieves state-of-the-art performance on all datasets and can even outperform some weakly-supervised approaches, demonstrating its effectiveness and generalizability.

==> wacv2022_SSCAP_ Self-supervised Co-occurrence Action Parsing for Unsupervised Temporal Action Segmentation/relatedwork.tex <==
\section{Related Work}
\label{section:relatedwork}



\textbf{Temporal action segmentation} is a task to classify each frame in an untrimmed video with a label of action. It is a key for understanding structures of complex activities. While current deep learning techniques~\cite{lin2019tsm,after-unet,Ji_2021_ICCV,feichtenhofer2016convolutional,Liu_2020_CVPR,li2021learning,cdg,ma2021transfusion,tran2015learning,gpa} have achieved great success on other action understanding tasks such as action recognition~\cite{i3d,feichtenhofer2019slowfast,yang2020temporal,wang2016temporal,zhou2018temporal,wang2018non,gmmhmm,zwicassp} and action detection~\cite{lin2018bsn,zhao2017temporal,xu2017r,hou2017tube}, temporal action segmentation is still far from being well-explored. Today's high performing solutions for temporal action segmentation require full frame-level supervision~\cite{mstcn,gcnactionseg,htk,bcn,lea2016segmental,lea2017temporal,ddxd}.
However, acquiring annotations on fine-grained sub-actions for each frame is expensive. To reduce the amount of labeled data needed,~\cite{sstda} proposes a domain adaptation approach based on self-supervised auxiliary tasks and achieves good performance. More recent works focus on developing weakly-supervised solutions: instead of having supervision for every frame, only the list (with order information)~\cite{firstunsuper,energyweaklyactionseg,nnviterbi,Richard_2017_CVPR,ding2018weakly,huang2016connectionist,chang2019d3tw} or the set (without order information)~\cite{actionsetscvpr2020,setViterbi,actionsetscvpr2018} of the sub-actions in each video are required during training. Other work uses script
or instructions for weak annotation~\cite{alayrac2016unsupervised}.
Unsupervised temporal action segmentation, which does not have any supervision signal per video, starts to receive growing interests these days, to further reduce the dependence on labeled data ~\cite{UnsuperProcLearn,cvpr2018,cvpr2019cnnrnn,kukleva2019unsupervisedtemporalembedding,vidalmata2020joint,JS,MNVALR}.  However, these solutions do not fully explore the self-supervised feature, do not take into account semantic correlations among sub-actions and the recurrence of sub-actions in some complex activity structures. The performance of them is still far from desired. 

%\textbf{Unsupervised temporal action segmentation} starts to receive growing interests these days, to further reduce the dependence on labeled data.~\cite{UnsuperProcLearn} builds a joint sequential subset selection method to produces a summary of the procedure key-steps in instructional videos.~\cite{cvpr2018} learns a function assigning sub-activity scores to frame features and models the distribution over sub-activity permutations by a Generalized Mallows Model.~\cite{cvpr2019cnnrnn} proposes a self-supervised predictive learning with recurrent neural networks (RNN) by utilizing features of adjacent frames to find the action boundaries.~\cite{kukleva2019unsupervisedtemporalembedding} proposes a combination of temporal embedding generated using a frame timestamp prediction network, feature clustering and Viterbi decoding for consistent frame-to-cluster assignment. However, these solutions do not take into account the semantic correlations among sub-actions and the re-occurrence of sub-actions in some complex activity structures.







\textbf{Self-supervised learning of visual representation} is a hot topic today, and has shown success in some of action understanding tasks~\cite{lstmunsupervisedfaeture,Deeo_Clustering,speednet,fernando2017self}.  Many different video properties have been used as supervision to build good representations, such as: cycle consistency between video frames \cite{xiaolongcvpr2019}; distinguishing between a video frame sequence and a shuffled version of it \cite{shufflelearn}; predicting the order of the shuffled clips \cite{cliporder}; solving space-time cubic puzzles \cite{spacetimecubicpuzzles}; classifying the speed of the video \cite{speednet,speednetMIT}; recognize the rotation of the video \cite{rotationet}. Another common task is predicting the future, either by predicting pixels of future frames \cite{motionnet}, or an embedding of a future video segment \cite{pdc}. While today's action segmentation solutions~\cite{mstcn,kukleva2019unsupervisedtemporalembedding,bcn} still mainly rely on hand-crafted features such as IDT~\cite{idt}, Fisher Vector (FV)~\cite{fishervector}, or pre-trained features such as I3D on Kinetics dataset~\cite{i3d}, we believe that introducing self-supervised methods in feature representation learning for unsupervised action segmentation can significantly boost the performance, as it can not only bring strong discriminative power to the features, but also bring a chance to improve the temporal characteristics of the features. 

